Experiments with Rich Regime Training for Deep Learning

In spite of advances in understanding lazy training, recent work attributes the practical success of deep learning to the rich regime with complex inductive bias. In this paper, we study rich regime training empirically with benchmark datasets, and find that while most parameters are lazy, there is always a small number of active parameters which change quite a bit during training. We show that re-initializing (resetting to their initial random values) the active parameters leads to worse generalization. Further, we show that most of the active parameters are in the bottom layers, close to the input, especially as the networks become wider. Based on such observations, we study static Layer-Wise Sparse (LWS) SGD, which only updates some subsets of layers. We find that only updating the top and bottom layers have good generalization and, as expected, only updating the top layers yields a fast algorithm. Inspired by this, we investigate probabilistic LWS-SGD, which mostly updates the top layers and occasionally updates the full network. We show that probabilistic LWS-SGD matches the generalization performance of vanilla SGD and the back-propagation time can be 2-5 times more efficient.

==> sections/prelim.tex <==
% \begin{table*}[t]
%     \centering
%     \caption{Summary of notations used in the paper.}
%     %\resizebox{.5\textwidth}{!}{
%     \begin{tabular}{cc}
%     \hline
% Mathematical Notation & Description\\
% \hline 
% $\theta \in \mathbb{R}^p$ & Model parameter \\
% $z \in \cZ$ & Sample \\
% $S = \{z_1, .., z_n\}$ & Training samples \\
% $\ell(\theta, z)$ & Loss \\
% $\cL_S(\theta) = \frac{1}{n}\sum_{i=1}^n \ell(\theta, z_i)$ & Empirical risk \\
% $\cL_\cP(\theta) = \mathbb{E}_{z\sim\cP} \ell(\theta, z)$ & Population risk\\
% $\nabla \ell(\theta, z)$ & Sample gradient\\
% $H(\theta) = \sum_{i=1}^n \nabla^2 \ell (\theta,z_i)$ & Empirical Hessian\\
% $t \in \{1,..., T\}$ & Iteration \\
% $B_t$ & Mini batch at iterate t\\
% $g\left(\mathbf{\theta}_{t}, B_{t}\right)=\frac{1}{\left|B_{t}\right|} \sum_{z_{i} \in B_{t}} \nabla \ell\left(\mathbf{\theta}_{t}, z_{i}\right)$ & Mini-batch gradient\\
% $\eta_t$ & Learning rate\\
% $d$ & Neural network depth\\
% $w$ & Neural network width (No. of hidden units per layer)\\
% $p$ & No. of Neural network parameters\\
% $n$ & No. of training samples\\
% $\varepsilon$ & \makecell{the top $\varepsilon \%$ parameters to keep while\\ the remaining $(100-\varepsilon) \%$ to be replaced by their initial values}\\
% $\gamma$ & \makecell{the top $\gamma \%$ parameters to be replaced by their initial values while\\ the remaining $(100-\varepsilon) \%$ to keep as they are at convergence}\\
% \hline
% \end{tabular}
% %}
% \end{table*}


Consider a parameterized neural network model, e.g., Feed-forward Neural Network with Relu activation (Relu-Net) and Convolutional Neural Network (Conv-Net). The model starts at parameter value $p^0$ and ends at parameter value $p^T$ after training for $T$ epochs.

A neural network with depth $d$ has $d-1$ hidden layers. 
We use $l_0$ to denote the input layer, $l_d$ to denote the output layer, and $l_i$ to denote the $i$ hidden layer in between.

We order the layers by their closeness to the input layer, we call the layers that are close to the input layer as bottom/lower layers, and the layers that are close to the output layer as top/upper layers. We use $w$ to denote the width of a Relu-Net or the number of channels of a Conv-Net.


